Explaining generalization in deep learning: progress and fundamental limits

This dissertation studies a fundamental open challenge in deep learning theory: why do deep networks generalize well even while being overparameterized, unregularized and fitting the training data to zero error? In the first part of the thesis, we will empirically study how training deep networks via stochastic gradient descent implicitly controls the networks' capacity. Subsequently, to show how this leads to better generalization, we will derive {\em data-dependent} {\em uniform-convergence-based} generalization bounds with improved dependencies on the parameter count. Uniform convergence has in fact been the most widely used tool in deep learning literature, thanks to its simplicity and generality. Given its popularity, in this thesis, we will also take a step back to identify the fundamental limits of uniform convergence as a tool to explain generalization. In particular, we will show that in some example overparameterized settings, {\em any} uniform convergence bound will provide only a vacuous generalization bound. With this realization in mind, in the last part of the thesis, we will change course and introduce an {\em empirical} technique to estimate generalization using unlabeled data. Our technique does not rely on any notion of uniform-convergece-based complexity and is remarkably precise. We will theoretically show why our technique enjoys such precision. We will conclude by discussing how future work could explore novel ways to incorporate distributional assumptions in generalization bounds (such as in the form of unlabeled data) and explore other tools to derive bounds, perhaps by modifying uniform convergence or by developing completely new tools altogether.

==> background.tex <==
\section{Overview of cluster storage systems}
Large-scale distributed storage systems such as the Google File System~\cite{ghemawat2003google}, Colossus, Amazon S3~\cite{amazons3}, Microsoft Azure~\cite{calder2011windows}, etc. are composed of multiple cluster storage systems (also called storage clusters). Each cluster is typically divided into multiple storage tiers, each with a distinct purpose, such as the caching tier (also known as the hot tier for short-lived or high-performance data), the primary storage tier (also known as the warm tier where the bulk of the data that is actively in use and has moderate churn resides), the archival tier (also known as the cold tier meant for backups), etc. Large-scale storage clusters can have anywhere between tens to hundreds of thousands of storage devices in their primary storage tier. Furthermore, most clusters in today's large-scale distributed systems are designed in a disaggregated manner, wherein the space on all the storage devices in the same tier is exposed as a single, large addressable storage pool~\cite{legtchenko2017understanding}. Data stored in such clusters is stored across a number of storage devices. In most such clusters, clients access any given device directly (via a storage network) or indirectly (via whichever networked storage-node it is attached to) after contacting a logically-separate metadata service that maintains data location and other information
% \footnote{For simplicity, we will use the terms ``device'' or ``disk'', even though a storage-node may contain multiple types of devices.}. 
While details vary, this basic architecture enables large and time-varying numbers of devices to be used effectively.

\subsection{Hard disk drives are the primary storage devices}
Owing to the economical price-point calculated in terms of dollars-per-terabyte (\$/TB), the primary storage tier of most of the large-scale storage clusters today is made up of hard disk drives (HDDs). Throughout this dissertation, any reference to a storage device or a disk implies a reference to a HDD. The storage capacity (space) of commonly used disks ranges from anywhere between 4TB--14TB. The price dynamics are unlikely to change drastically in the foreseeable future, ensuring that the bulk of the bytes in large-scale distributed systems and cloud computing platforms will continue to be stored on HDDs~\cite{brewer-keynote, brewer2016disks}. 

\subsection{Disk failures are common}
In large-scale storage clusters disk failures happen all the time~\cite{ghemawat2003google,schroeder2007disk}. In fact, modern distributed storage systems are designed for failures, which means that they treat failures as the norm, and not an exception from the norm~\cite{ghemawat2003google, patterson2002recovery, shvachko2010hadoop}.
Storage devices exhibit two kinds of failures: \textit{partial failures} and \textit{fail-stops} (complete failures). Partial failures might involve a particular read or write failing because of a sector error or checksum failure. The disk as a whole is still functional, and usually it remaps failed sectors to spare locations in order to continue operation. In the case of fail-stop, the disk stops functioning altogether. This dissertation focuses on data redundancy optimizations for fail-stop failures where all the data from a disk is permanently lost when the disk fails.

% \subsection{Storage clusters have heterogeneous disk populations}
% \rashmi{Is this subsection needed here? Takes away some of the punch. Can come in third section?}
% A per-acquisition optimization of which make/model to acquire (such as targeting the lowest \$/TB option available at the time, or requiring the largest capacity disks) leads to a diverse population of disks in any given large-scale storage cluster. The storage clusters we evaluated had between 3--10 makes/models of disks deployed over a span of a few years. As disks age, or as technology advances, it is common to retire or decommission older disk models and replace them with newer, more advanced variants. Chapter~\ref{chapter:insights} has more details about the composition of the different clusters evaluated as a part of this research.

\section{Data reliability is achieved using data redundancy} \label{sec:background_redundancy}
Data redundancy is the most common approach to protect against permanent data loss amongst continuous disk failures~\cite{ghemawat2003google, huang2012erasure, pinheiro2007failure, backblaze, rashmi2013solution, rashmi2015hitchhiker,sathiamoorthy2013xoring}.
% , it is important that there is enough data redundancy such that disk failures do not result in permanent data loss. 
There are two common ways of performing data redundancy.

% \subsubsection{Different notions of reliability}
% There are two ways of quantifying data reliability.

% \textbf{Durability.}
% Durability is the measure of long-term data protection. It reflects the ability to recover the data  Durability is measured in terms of \textit{mean time to data loss}, i.e. when data is stored redundantly, how much time does it take (on average) before enough copies of data are lost for there to permanent data loss~\cite{gibson1992redundant}.

% \textbf{Availability.}
% \sk{define availability and mention its metric}

% This research focuses on durability. \sk{give more details about why we focus only on durability, and that adding availability can be done on the same lines.}

\subsection{Replication}
% There are numerous methods of data redundancy. The two most common forms are replication and erasure coding.
Replication involves creating exact copies of the data on different disks as backup. Usually, data is either duplicated (2-way replicated) or triplicated (3-way replicated). Replication not only makes the data more durable, but also improves its availability since the redundant copies of the data can be used to service reads in parallel.

The degraded mode read algorithm (i.e. the algorithm followed in case one of the disks on which data is stored fails) for replication is very straightforward. The other copies of data are referenced until the lost copy is replenished. There is a background process that continuously monitors if data is under-redundant, and replenishes lost copies using the healthy copies of data that are stored on other disks.

% Replication is the preferred method of redundancy for hot data owing to its simple degraded read mode algorithm and no expensive processing of data when referencing its redundant copies. The disadvantage of replication is its high storage cost, where $k$-way replication requires storage capacity that is $k\times$ the size of the data.
For hot data with certain access patterns, replication may be viewed as the right option for performance, with the replication factor chosen to provide sufficient reliability. But, of course, the cost consequence is a doubling or tripling of the number of disks needed. This makes replication infeasible for majority of the data in modern storage clusters.

\subsection{Erasure coding}\label{subsec:background.ec}
Erasure code is a more space-efficient redundancy mechanism compared to replication. For erasure coding a file, it is first broken into identically sized chunks of data where each chunk is at most a few MBs. Every $k$ chunks of data are then combined with $n-k$ identically sized parity chunks to form an $n$ chunk \textit{stripe}. For the popularly used maximum distance separable (MDS) codes, any $k$ chunks can be used to recover any of the $n$ chunks. In this dissertation we use the notation $k$-of-$n$ scheme to indicate an erasure code with $k$ data chunks and $n-k$ parity chunks per stripe. $k$ and $n$ are also known as the ``dimension'' and the ``length'' of the erasure code. Erasure codes can also be denoted using the $(n, k)$ notation. Both these notations follow the standard notation employed in the coding theory literature. Replication can also be denoted using this notation. For example, 3-replication can be denoted as a 1-of-3 erasure code. Although the description of the notation applies only to ``systematic'' codes, and most of the erasure codes employed in storage systems are indeed systematic. We will use the $k$-of-$n$ notation in this dissertation.

The degraded mode read algorithm for erasure coding is more costly and complex compared to that of replication. When a read is requested to a chunk that is missing because the disk on which it was stored has failed, it triggers a process called data reconstruction. Data reconstruction for MDS codes) involves reading any $k$ of the remaining chunks from the stripe that the missing chunk belongs to, after which the missing data is reconstructed using the combination of parity and data chunks that are read.
% , to a common location (either the client of one of the server nodes). 
% Then, the missing data is reconstructed using the combination of parity and data chunks that are read. 
The reconstructed data is then provided to the requesting client. Similar to replication, there is a background monitor process that keeps checking for under-redundant data and issues reconstructions proactively without being triggered by client reads.

It is increasingly common, in large-scale systems, to use erasure-coding (with $k>1$) for bulk and colder data. With erasure-coding, space efficiency ($\frac{n}{k}$) for tolerating a given number of failures is better. But, additional considerations arise regarding the amount of work involved in recovering from a device failure---since $k$ remaining chunks must be read to reconstruct each lost chunk, too high a $k$ will result in more work than desired and, potentially, full recovery time that is too long. Schemes like 6-of-9 and 10-of-14 have been reported for real deployments~\cite{facebookECsavings2010, fikes2010storage, ford2010availability, rashmi2013solution, rashmi2015hitchhiker, sathiamoorthy2013xoring}, and Backblaze reports use of 17-of-20~\cite{backblazeerasurecoding}.
% \sk{note to self: we currently test backblaze for 6-of-9 default. re-run for 17-of-20 default and see what it looks like. if numbers are bad, can go wider in max stripe because this is cold data. re-run Google for 8-of-12 default and see what that looks like.}

% For any $k$-of-$n$ scheme, the storage overhead is given by the ratio $\frac{n}{k}$. Popularly used erasure codes in large-scale storage clusters are 6-of-9 or 10-of-14~\cite{facebookECsavings2010, fikes2010storage, ford2010availability}, which have a storage overhead of $1.5\times$ and $1.4\times$ respectively. Thus, commonly used erasure coding schemes are significantly cheaper than commonly used replication schemes, but they come with the caveat of IO-heavy and time-consuming degraded mode reads. This makes erasure coding more suitable for warm or cold data which is not performance-critical, but is the data that occupies bulk of the bytes in a storage cluster.

\subsection{Metrics of data reliability}
\subsubsection{Annualized failure rate (\afr{})}\label{sec:afr}
\textit{Annualized failure rate (\afr{})} is the standard metric used to describe a disk's fail-stop rate~\cite{cole2000estimating}.
%all the data on the disk is instantly unreadable.}.
%, because the disk has failed beyond repair.}. 
% \sk{There's a Seagate blog-like reference about using AFR as the standard. I checked that Bianca and Garth's paper also cited something similar for AFR. Would that work?} \rv{Yes.} 
As the name suggests, it is the expected percentage of disks that will fail-stop in a given year from a population of disks. We calculate \afr{} using the following formula:
\begin{equation}\label{eqn:afr}
AFR\;(\%) = \frac{f_d}{n_1+n_2+\ldots+n_d}\times365\times100
\end{equation}
where $f_d$ is the number of disks failed in $d$ days (a sliding window of typically 30 to 60 days; used to eliminate the jitter observed in instantaneous failure rates) and $n_i$ is the number of disks operational during day $i$. Next, we will show how the \afr{} is used in the reliability calculation of a redundancy scheme.

\begin{figure}
    \centering
    \begin{tikzpicture}[]
        % Draw the states
        \node[state]             (0) {\textbf{0}};
        \node[state, right=of 0] (1) {\textbf{1}};
        \node[state, right=of 1] (d) {\textbf{\dots}};
        \node[state, right=of d] (s) {\textbf{n-k}};
        \node[state, right=of s] (t) {\textbf{DL}};
 
        % Connect the states with arrows
        \draw[every loop]
            (0) edge[bend left, auto=left] node {$n\lambda$} (1)
            (1) edge[bend left, auto=left] node {$\mu$} (0);
        \draw[every loop]
            (1) edge[bend left, auto=left] node {$(n-1)\lambda$} (d)
            (d) edge[bend left, auto=left] node {$\mu$} (1);
        \draw[every loop]
            (d) edge[bend left, auto=left] node {$(n-k-1)\lambda$} (s)
            (s) edge[bend left, auto=left] node {$\mu$} (d);
        \draw[every loop]
            (s) edge[bend left, auto=left] node {$(n-k)\lambda$} (t);
            % (t) edge[bend left, auto=left] node {$\mu$} (d);
    \label{fig:mttdl}
    \end{tikzpicture}
    \caption{Continuous-time Markov chain used to calculate the MTTDL of a $k$-of-$n$ erasure coded stripe.}
    \label{fig:k-of-n-mttdl}
\end{figure}

\subsubsection{Mean time to data loss (\mttdl{})}\label{sec:reliability}
The standard metric used for reliability of data is \textit{mean time to data loss} (\mttdl{}). \mttdl{} is calculated based on two rates -- \textit{mean time to failure} (MTTF) and \textit{mean time to repair} (\mttr{})~\cite{patterson1988case, trivedi2002probability}. MTTF is a function of the disk's \afr{}, while the \mttr{} is the time it takes to reconstruct the lost data from the failed disk. In a large-scale cluster storage system, multiple copies of the data exist, that too on distinct disks. Thus, the effort of reconstructing the lost data of a failed disk is shared by numerous disks, which can be so efficient that the time it takes to detect and take action upon a failed disk (approximately 15 minutes~\cite{ford2010availability,rashmi2013solution,rashmi2015hitchhiker}) dominates the time taken to reconstruct all of its data~\cite{ford2010availability}. This decouples the \mttr{} of the disk from its storage capacity. Thus, in large cluster storage systems, the data reliability is only a function of the disk's MTTF (which is a function of its \afr{}).

When using erasure coding for fault tolerance, \mttdl{} is calculated at a stripe granularity. A stripe is a set of fixed sized chunks that include both data and parity chunks as explained in \S\ref{subsec:background.ec}. Figure~\ref{fig:k-of-n-mttdl} shows the continuous-time Markov chain that is typically used for calculating the \mttdl of a $k$-of-$n$ stripe. Each state in the Markov chain represents number of failed chunks in the stripe, starting with \textbf{0} and ending with \textbf{DL} to denote permanent data loss. Each chunk of a stripe is stored on a separate disk, and for the purpose of calculating the \mttdl, all disks are assumed to fail independent of each other. This simplifies the \mttdl calculation since we can assume that disk failures and repairs are distributed exponentially (in this case with a failure rate of $\lambda$). Each arrow to the right indicates failure rate, i.e. $\frac{1}{MTTF}$ whereas each arrow to the left indicates repair rate, i.e. $\frac{1}{MTTR}$. The time to reach from state \textbf{0} to state \textbf{DL} is the \mttdl, and is usually denoted in tens-of-thousands to millions of hours.
% \newline
% \newline
% \begin{center}

% \end{center}

% \section{Redundancy scheme selection}
% Generally, administrators determine the redundancy scheme to be used based on several factors, including cost, performance, and data reliability. 
% For hot data with certain access patterns, replication may be viewed as the right option for performance, with the replication factor chosen to provide sufficient reliability. But, of course, the cost consequence is a doubling or tripling of the number of devices needed.
% Thus, it is increasingly common, in large-scale systems, to use erasure-coding (with $k>1$) for bulk and colder data. With erasure-coding, space efficiency ($\frac{n}{k}$) for tolerating a given number of failures is better. But, additional considerations arise regarding the amount of work involved in recovering from a device failure---since $k$ remaining chunks must be read to reconstruct each lost chunk, too high a $k$ will result in more work than desired and, potentially, full recovery time that is too long. Schemes like 6-of-9 and 10-of-14 have been reported for real deployments~\cite{ford2010availability, rashmi2013solution, rashmi2015hitchhiker, sathiamoorthy2013xoring}, and Backblaze reports use of 17-of-20~\cite{backblazeerasurecoding}.
% \sk{note to self: we currently test backblaze for 6-of-9 default. re-run for 17-of-20 default and see what it looks like. if numbers are bad, can go wider in max stripe because this is cold data. re-run Google for 8-of-12 default and see what that looks like.}

% For long-term storage, protecting data from loss is a critical constraint. Given the \mttdl and per-make/model \afr and \mttr, the subset of redundancy scheme options that would achieve a target \mttdl{} can be identified; the final selection can be based on the other considerations.

% \textbf{Distributed storage architecture and life cycle.}
% Scalable distributed storage systems, broadly speaking, spread data
% across a large number of storage devices.
% In most such systems, clients access any given device directly (via a storage network)
% or indirectly (via whichever networked storage-node it is attached to)
% after contacting a logically-separate metadata service that maintains data
% location and other information.\footnote{For simplicity, the discussion
% below will discuss things in terms of ``device'' or ``disk'', even though a storage-node
% may contain multiple devices.}
% While details vary, this basic architecture enables large and time-varying
% numbers of devices to be used effectively.


% %\greg{"grow-with-the-business" incremental vs. "one-cluster-within-the-warehouse" batch ?}

% \begin{comment}
% In practice, most large-scale instances of such systems are deployed
% incrementally rather than all at once.
% That is, devices are added over time, as capacity and performance
% demands grow and as older devices are replaced.
% For example, addition of 2--5\% of the device count each month would
% be consistent with rolling 4-year refresh of devices combined
% with reasonable additions for growth and failed device replacement.
% For a system like the one used for the Backblaze Internet backup service,
% with 100,000 devices, this means 1000s of devices per month; for
% large cloud/service companies, the numbers are much higher.
% \end{comment}

% In most large-scale instances (10s to 100s of thousands of devices) of such systems, storage devices of different ages of different makes/models are used.
% A mix of makes/models is used because
% the most cost-effective choice changes over time and, at
% large-scale, reliance on a single vendor/product-line can be undesirable.
% Different device ages arise because devices are added over time as capacity and performance demands grow and as older devices are replaced.
% In some cases, such as for the Backblaze Internet backup service, relatively smooth incremental growth is seen over its 6-year lifetime, due to a steady trickle of 10s/100s-device deployments.
% In other cases, such as the Google clusters, most of the growth occurs in larger steps, each representing deployments of 10s of 1000s of devices in a few days.

% %\greg{should we try to do a simple figure to illustrate the two patterns, point forward to the detailed eval graphs, or leave it as "good enough in brief text" here?}
% %\greg{if going for illustration, is there a way to combine it with the unknown but wished-for Sec3 figure?}\\
% %\rashmi{We need figure(s): one for Backblaze and one for Google. I was thinking about needing figures and I encountered your comment! It would be great to combine with the figure needed in Section 3. Let us drop the idea of using "toy" example there and try to incorporate with this figure.}


% Since device failures are inevitable in large-scale systems, data is
% stored redundantly.
% Using $k$-of-$n$ erasure coding ($n$-way replication being 1-of-$n$)
% as a general example, where $k$ data
% chunks are coupled with $n-k$ ``parity'' chunks to form a stripe.
% Rather than tying devices into tight redundancy groups, 
% % \jason{why do we need quote for parity?} 
% as in traditional
% RAID system designs, most systems decluster redundancy to simplify scaling and 
% % \jason{what is systems decluster?}
% spread load when a device fails. 
% That is, most systems assign any given stripe to $n$ devices
% chosen pseudo-randomly (with some constraints, like ``not same rack''.
% % \Saurabh{is this too colloqial? How about ``in accordance with fault domains"}\greg{I'm a huge believer in clarity/ease-of-read over formality, in things other than math or algorithm detailing where formality augments clarity.}).
% As a result, many sets of $n$ devices within the system will collectively
% hold at least one full stripe.

\section{Characterizing disk reliability over lifetime: the disk bathtub curve} \label{sec:background_bathtub}
% \sk{describe the disk bathtub curve and what it means for data reliability.}
Disk reliability varies over its lifetime as shown in Figure~\ref{fig:canonical_bathtub_background}. When the disk is in its infancy, it suffers from \textit{infant mortality}. Infant mortality is also referred to as ``burn-in'' failure rate, and is an increased failure rate usually triggered due to new environment, workload pattern, etc. Eventually the disk \afr plateaus into a low, stable failure rate regime. This regime is called \textit{useful life}. Infancy lasts 3--5 months whereas useful life lasts 3--4 years. Once the disk is heavily used for approximately 4 years, it suffers from another phase of high \afr similar to infancy. This phase of life is called \textit{wearout}. When a disk is old enough to be considered to be in its wearout phase, it is usually decommissioned before it fails. This way the data on the disk can be copied over to other disks rather than performing the IO and time-intensive data reconstruction once the disk fails. Moreover, during reconstruction the data is vulnerable to being permanently lost if many such disks fail together. \csknew{Chapters~\ref{chapter:heart} and~\ref{chapter:pacemaker} contains various \afr curves from the different disk makes/models that we have analyzed to facilitate \dadaptred.}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{heart/figures/2018-09-25/bathtub.pdf}
\caption{The disk hazard curve (also known as the bathtub curve) showing disk reliability over its lifetime.}
\label{fig:canonical_bathtub_background}
\end{figure}

\section{Scheme selection problem for scalable storage} \label{sec:background_same_redundancy}
Generally, administrators determine the redundancy scheme to be used based on several factors, including cost, performance, and data reliability. For long-term storage, protecting data from loss is a critical constraint. Given the \mttdl and per-make/model \afr and \mttr, the subset of redundancy scheme options that would achieve a target \mttdl{} can be identified; the final selection can be based on the other considerations. Unfortunately, this simple-sounding approach doesn't work well for large-scale systems. 
% \suhas{Start the sentence with something else and then lead to "unfortunately". Otherwise it seems like a break in the reading flow.}
Specifically, the \mttdl{} equations rely on devices all conforming to the same stationary \afr{} value and the administrator knowing that value; neither of which are true.
% \suhas{Two "unfortunately" to talk about the same problem? Use some other negative?}
\csknew{Although it may be tempting to use \afr{} values taken from manufacturer's specifications, studies have shown that failures rates observed in practice often do not match those~\cite{schroeder2007disk}.
More importantly, \afr{} values vary significantly between makes/models as we will see in Chapters~\ref{chapter:heart}--\ref{chapter:pacemaker}, and for devices of different ages as described in \S\ref{sec:background_bathtub}. Given these two dimensions of \afr heterogeneity, using a single redundancy scheme for all disks, and throughout each disk's life is often wasteful, but can also be dangerous. In order to improve data safety and cost-effectiveness a cluster storage system needs to rethink its ``one-scheme-fits-all'' redundancy mechanism and employ a more sophisticated approach that takes into account the aforementioned dimensions of \afr hetereogeneity.}
% ~\cite{schroeder2007disk, ma2015raidshield, pinheiro2007failure}. 
% Deployed disks roughly age through three phases of life: infancy, when the failure rate may be high and unstable; useful life, when the failure rate is lower and more stable; and wearout, where the failure rate climbs and grows more unstable \csknew{as described in \S\ref{sec:background_bathtub} and shown in Chapters~\ref{chapter:heart} and \ref{chapter:pacemaker} via practically observed \afr curves.} %\suhas{Is this required here? It adds no extra info to the topic in this paragraph.}
% Since large-scale systems include mixes of makes/models and of 
% ages,
% % \footnote{Deployed disks roughly go through three phases of life: infancy, when the failure rate may be high and unstable; useful life, when the failure rate is lower and more stable; and wearout, where the failure rate climbs and grows more unstable. \rashmi{We use the terms infancy and wearout far too often in the later part of the paper to make this a footnote. I think this needs to be in the main text.}},
% no single stationary \afr{} value exists for use in \mttdl{} equations.

% \csknew{HAVE TO CAREFULLY THINK ABOUT THIS}

% The \mttdl{} equations can still be used to guide decisions, as long as a sufficiently high \afr{} value is used.
% For example, if the highest \afr{} value possible for any deployed make/model at any age allowed (before decommissioning) is used, the computed \mttdl{} will be a lower bound.
% Unfortunately, the range of possible \afr{} values in a deployed system is generally quite large~\cite{schroeder2016flash,ma2015raidshield,pinheiro2007failure,kadekodi2019cluster}.  For example, we observe the range to be well over an order of magnitude in the NetApp and Google logs discussed later, from rare occurrences of double-digit \afr{s} to more commonly observed low single digit \afr{s}. Since the overall average is much closer to the lower end of the \afr range, the highest value is a very conservative over-estimate for most of the devices. 
% \suhas{add ", leading decision-makers to use excessive redundancy." and omit "resulting MTTLs are very loose". The paragraph already starts with that statement.}
% The resulting \mttdl{}s are thus very loose lower bounds, leading decision-makers to use excessive redundancy.
% \Saurabh{I find this paragraph confusing because we map \afr{} to \mttdl{} and vary one to show how bad the other is, and that I personally find confusing. Can we simplify this?}

% Nonetheless, we are told by admins of large storage deployments that such approaches, and other ad hoc approaches to conservative over-protection, are the norm.
% Such approaches are problematic in two significant ways.
% First, they result in much higher cost overheads than might otherwise be necessary.
% Second, and more insidious, they are still risky, because it is unclear (until too late) how conservative one needs to be.
%---just because administrators believe they are being conservative enough, given cost and performance concerns, they will only know in retrospect.

